Support and Invertibility in Domain-Invariant Representations

Learning domain-invariant representations has become a popular approach to unsupervised domain adaptation and is often justified by invoking a particular suite of theoretical results. We argue that there are two significant flaws in such arguments. First, the results in question hold only for a fixed representation and do not account for information lost in non-invertible transformations. Second, domain invariance is often a far too strict requirement and does not always lead to consistent estimation, even under strong and favorable assumptions. In this work, we give generalization bounds for unsupervised domain adaptation that hold for any representation function by acknowledging the cost of non-invertibility. In addition, we show that penalizing distance between densities is often wasteful and propose a bound based on measuring the extent to which the support of the source domain covers the target domain. We perform experiments on well-known benchmarks that illustrate the short-comings of current standard practice.

==> app_ptl.tex <==
%
% PTL Bounds
%

\section{Bounds under PTL}
\citet{courty2017joint} gave a bound on the adaptation under covariate \emph{and} label shift and the assumption of probabilistic transfer Lipschitzness. As a tool, they used the Wasserstein distance between the joint distributions of features and labels in the source and target respectively. As we only have a shift in covariates, we adapt their bound to the case without label shift below, slightly changing its form.

\begin{thmthm}
Let $\cH \subset \{\cX \rightarrow \cY\}$ be an hypothesis class over a metric feature space $(\cX, d)$ with $\cY$ the label space. Let $f\in \cH$ and domains $p(x,y)$, $q(x,y)$ be defined over $\cX$. We observe $N_s$ labeled samples from $p$ and $N_t$ unlabeled samples from $q$. Then, let $\Pi^* = \argmin_{\pi} W_1(p,q)$. \fxfatal{Is this what we need?} Let $f^* \in \cH$ be a labelling function that satisfies PTL w.r.t. $\Pi^*$ and that minimizes the joint error $R_s(f^*) + R_t(f^*)$ w.r.t all functions in $\cH$ PTL w.r.t. $\Pi^*$. Further assume that $\forall x,x' \in \cX : \|x - x'\| \leq K$ and as a result, $|f^*(x) - f^*(x')| \leq M$. Let $\ell$ be a symmetric and $k$-Lipschitz loss function on $\cY$.
\end{thmthm}
\begin{proof}
By symmetry of the loss, we have
\begin{equation}
R_t(f) \leq R_t(f, f^*) + R_t(f^*)
\end{equation}
Then,
\begin{align}
R_t(f, f^*) & = R_t(f, f^*) - R_s(f, f^*) + R_s(f, f^*) \\
& \leq R_t(f,f^*) - R_s(f, f^*) + R_s(f) + R_s(f^*)
\end{align}
Further,
\begin{align}
R_t(f,f^*) - R_s(f, f^*) & \leq \left| \int_{\cX} \ell(f(x), f^*(x))(dp - dq) \right| \\
& \leq  \int_{{\cX}^2} \left| \ell(f(x), f^*(x)) - \ell(f(x'), f^*(x'))\right| d\Pi^*(x, x') \\
& \leq  \int_{{\cX}^2} k\left|f^*(x) - f^*(x')\right| d\Pi^*(x, x') \\
& = W_1(p(x), q(x)) + kM\phi(\lambda)
\end{align}
All in all,
$$
R_t(f) \leq R_s(f) +  W_1(p(x), q(x)) + R_s(f^*) + R_t(f^*) + kM\phi(\lambda)
$$
\end{proof}


==> consistency.tex <==
%
% Impossibility
%

